Vision-based Oxy-fuel Torch Control for Robotic Metal Cutting

The automation of key processes in metal cutting would substantially benefit many industries such as manufacturing and metal recycling. We present a vision-based control scheme for automated metal cutting with oxy-fuel torches, an established cutting medium in industry. The system consists of a robot equipped with a cutting torch and an eye-in-hand camera observing the scene behind a tinted visor. We develop a vision-based control algorithm to servo the torch's motion by visually observing its effects on the metal surface. As such, the vision system processes the metal surface's heat pool and computes its associated features, specifically pool convexity and intensity, which are then used for control. The operating conditions of the control problem are defined within which the stability is proven. In addition, metal cutting experiments are performed using a physical 1-DOF robot and oxy-fuel cutting equipment. Our results demonstrate the successful cutting of metal plates across three different plate thicknesses, relying purely on visual information without a priori knowledge of the thicknesses.

==> meta/biographies.tex <==
% CROP/RESIZE BIO PHOTOS TO BE 1.00:1.25 RATIO
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./img/bio_james.jpg}}]{James Akl} is currently pursuing the Ph.D. degree in Robotics Engineering at Worcester Polytechnic Institute, Worcester, MA, USA, with the Manipulation and Environmental Robotics Laboratory working on robotic metal scrap recycling. He received the B.E. degree in Mechanical Engineering and the Minor degree in Mathematics from the Lebanese American University, Byblos, Lebanon, in 2019.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./img/bio_fadi.jpg}}]{Fadi Alladkani}
received the B.E. degree in Mechanical Engineering from the Lebanese American University, Byblos, Lebanon, in 2019. He is currently pursuing the Ph.D. degree in Robotics Engineering at Worcester Polytechnic Institute, Worcester, MA, USA, with the Manipulation and Environmental Robotics Laboratory working on robotic waste sorting and ensemble learning for grasping.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./img/bio_berk.jpg}}]{Berk Calli}
is an Assistant Professor in the Robotics Engineering Department and in the Computer Science Department at
Worcester Polytechnic Institute (WPI) where he directs the Manipulation \& Environmental Robotics Laboratory. His main research focus is robotic manipulation and its applications in various domains such as waste and metal recycling, assistive technologies, and within-hand manipulation. His lab develops manipulation algorithms by combining techniques from computer vision, control theory, and machine learning. He also works on facilitating performance quantification methods for robotic manipulation, and is a founder of the Yale-CMU-Berkeley (YCB) benchmarking project, which provides a platform for the robotic manipulation community to develop and share benchmarking protocols. Prior to WPI, he was a postdoctoral researcher at Yale University's GRAB Lab, where he worked on vision-based dexterous manipulation with underactuated robotic hands. He received the Ph.D. degree at Delft University of Technology in The Netherlands, where he worked on active sensing aimed at increasing success rates of robotic grasping algorithms.
\end{IEEEbiography}

==> meta/notes/pkgs.tex <==
\usepackage{blindtext}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% *** FROM CASE MANUSCRIPT *** %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \usepackage{soul} % for text highlighting; remove once done
% \usepackage[vlined,ruled]{algorithm2e}
% \SetKwProg{Fn}{Function}{}{}
% \usepackage{cite}
% \usepackage{amsmath,amssymb,amsfonts}
% \usepackage{algorithmic}
% %\usepackage{algorithm}
% % \usepackage{graphicx}
% \usepackage{textcomp}
% \usepackage{xcolor}
% \usepackage{gensymb}
% \usepackage[utf8]{inputenc}
% \usepackage{array}
% \usepackage{wrapfig}
\usepackage{multirow}
% \usepackage{tabu}
% \usepackage{fullpage}
% \usepackage{times}
% \let\labelindent\relax % disables error-causing macro defined in IEEE .cls files
% \usepackage{enumitem,kantlipsum}
% %\usepackage{algpseudocode}
% \usepackage{fancyhdr,amsmath,amssymb}
% \usepackage[ruled,vlined]{algorithm2e}
% % \include{pythonlisting}
% % \usepackage[showframe]{geometry}
% \usepackage{lipsum}
% \usepackage{multicol}
% \usepackage{hyperref}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% *** FROM T-ASE TEMPLATE *** %%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% *** CITATION PACKAGES ***
\usepackage{blindtext}
\usepackage{cite}

% *** GRAPHICS RELATED PACKAGES ***
\ifCLASSINFOpdf
  \usepackage[pdftex]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../pdf/}{../jpeg/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.pdf,.jpeg,.png}
\else
  % or other class option (dvipsone, dvipdf, if not using dvips). graphicx
  % will default to the driver specified in the system graphics.cfg if no
  % driver is specified.
  % \usepackage[dvips]{graphicx}
  % declare the path(s) where your graphic files are
  % \graphicspath{{../eps/}}
  % and their extensions so you won't have to specify these with
  % every instance of \includegraphics
  % \DeclareGraphicsExtensions{.eps}
\fi
% graphicx was written by David Carlisle and Sebastian Rahtz. It is
% required if you want graphics, photos, etc. graphicx.sty is already
% installed on most LaTeX systems. The latest version and documentation
% can be obtained at: 
% http://www.ctan.org/pkg/graphicx
% Another good source of documentation is "Using Imported Graphics in
% LaTeX2e" by Keith Reckdahl which can be found at:
% http://www.ctan.org/pkg/epslatex
%
% latex, and pdflatex in dvi mode, support graphics in encapsulated
% postscript (.eps) format. pdflatex in pdf mode supports graphics
% in .pdf, .jpeg, .png and .mps (metapost) formats. Users should ensure
% that all non-photo figures use a vector format (.eps, .pdf, .mps) and
% not a bitmapped formats (.jpeg, .png). The IEEE frowns on bitmapped formats
% which can result in "jaggedy"/blurry rendering of lines and letters as
% well as large increases in file sizes.
%
% You can find documentation about the pdfTeX application at:
% http://www.tug.org/applications/pdftex

% *** MATH PACKAGES ***
\usepackage{amsmath}
% Note that the amsmath package sets \interdisplaylinepenalty to 10000
% thus preventing page breaks from occurring within multiline equations. Use:
%\interdisplaylinepenalty=2500
% after loading amsmath to restore such page breaks as IEEEtran.cls normally
% does. amsmath.sty is already installed on most LaTeX systems. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/amsmath

% *** SPECIALIZED LIST PACKAGES ***
\usepackage{algorithmic}
\usepackage[vlined,ruled]{algorithm2e}

% *** ALIGNMENT PACKAGES ***
\usepackage{array}
% Frank Mittelbach's and David Carlisle's array.sty patches and improves
% the standard LaTeX2e array and tabular environments to provide better
% appearance and additional user controls. As the default LaTeX2e table
% generation code is lacking to the point of almost being broken with
% respect to the quality of the end results, all users are strongly
% advised to use an enhanced (at the very least that provided by array.sty)
% set of table tools. array.sty is already installed on most systems. The
% latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/array

% IEEEtran contains the IEEEeqnarray family of commands that can be used to
% generate multiline equations as well as matrices, tables, etc., of high
% quality.

% *** SUBFIGURE PACKAGES ***
%\ifCLASSOPTIONcompsoc
%  \usepackage[caption=false,font=normalsize,labelfont=sf,textfont=sf]{subfig}
%\else
%  \usepackage[caption=false,font=footnotesize]{subfig}
%\fi
% subfig.sty, written by Steven Douglas Cochran, is the modern replacement
% for subfigure.sty, the latter of which is no longer maintained and is
% incompatible with some LaTeX packages including fixltx2e. However,
% subfig.sty requires and automatically loads Axel Sommerfeldt's caption.sty
% which will override IEEEtran.cls' handling of captions and this will result
% in non-IEEE style figure/table captions. To prevent this problem, be sure
% and invoke subfig.sty's "caption=false" package option (available since
% subfig.sty version 1.3, 2005/06/28) as this is will preserve IEEEtran.cls
% handling of captions.
% Note that the Computer Society format requires a larger sans serif font
% than the serif footnote size font used in traditional IEEE formatting
% and thus the need to invoke different subfig.sty package options depending
% on whether compsoc mode has been enabled.
%
% The latest version and documentation of subfig.sty can be obtained at:
% http://www.ctan.org/pkg/subfig

% *** FLOAT PACKAGES ***
%\usepackage{fixltx2e}
% fixltx2e, the successor to the earlier fix2col.sty, was written by
% Frank Mittelbach and David Carlisle. This package corrects a few problems
% in the LaTeX2e kernel, the most notable of which is that in current
% LaTeX2e releases, the ordering of single and double column floats is not
% guaranteed to be preserved. Thus, an unpatched LaTeX2e can allow a
% single column figure to be placed prior to an earlier double column
% figure.
% Be aware that LaTeX2e kernels dated 2015 and later have fixltx2e.sty's
% corrections already built into the system in which case a warning will
% be issued if an attempt is made to load fixltx2e.sty as it is no longer
% needed.
% The latest version and documentation can be found at:
% http://www.ctan.org/pkg/fixltx2e

%\usepackage{stfloats}
% stfloats.sty was written by Sigitas Tolusis. This package gives LaTeX2e
% the ability to do double column floats at the bottom of the page as well
% as the top. (e.g., "\begin{figure*}[!b]" is not normally possible in
% LaTeX2e). It also provides a command:
%\fnbelowfloat
% to enable the placement of footnotes below bottom floats (the standard
% LaTeX2e kernel puts them above bottom floats). This is an invasive package
% which rewrites many portions of the LaTeX2e float routines. It may not work
% with other packages that modify the LaTeX2e float routines. The latest
% version and documentation can be obtained at:
% http://www.ctan.org/pkg/stfloats
% Do not use the stfloats baselinefloat ability as the IEEE does not allow
% \baselineskip to stretch. Authors submitting work to the IEEE should note
% that the IEEE rarely uses double column equations and that authors should try
% to avoid such use. Do not be tempted to use the cuted.sty or midfloat.sty
% packages (also by Sigitas Tolusis) as the IEEE does not format its papers in
% such ways.
% Do not attempt to use stfloats with fixltx2e as they are incompatible.
% Instead, use Morten Hogholm'a dblfloatfix which combines the features
% of both fixltx2e and stfloats:
%
% \usepackage{dblfloatfix}
% The latest version can be found at:
% http://www.ctan.org/pkg/dblfloatfix

%\ifCLASSOPTIONcaptionsoff
%  \usepackage[nomarkers]{endfloat}
% \let\MYoriglatexcaption\caption
% \renewcommand{\caption}[2][\relax]{\MYoriglatexcaption[#2]{#2}}
%\fi
% endfloat.sty was written by James Darrell McCauley, Jeff Goldberg and 
% Axel Sommerfeldt. This package may be useful when used in conjunction with 
% IEEEtran.cls'  captionsoff option. Some IEEE journals/societies require that
% submissions have lists of figures/tables at the end of the paper and that
% figures/tables without any captions are placed on a page by themselves at
% the end of the document. If needed, the draftcls IEEEtran class option or
% \CLASSINPUTbaselinestretch interface can be used to increase the line
% spacing as well. Be sure and use the nomarkers option of endfloat to
% prevent endfloat from "marking" where the figures would have been placed
% in the text. The two hack lines of code above are a slight modification of
% that suggested by in the endfloat docs (section 8.4.1) to ensure that
% the full captions always appear in the list of figures/tables - even if
% the user used the short optional argument of \caption[]{}.
% IEEE papers do not typically make use of \caption[]'s optional argument,
% so this should not be an issue. A similar trick can be used to disable
% captions of packages such as subfig.sty that lack options to turn off
% the subcaptions:
% For subfig.sty:
% \let\MYorigsubfloat\subfloat
% \renewcommand{\subfloat}[2][\relax]{\MYorigsubfloat[]{#2}}
% However, the above trick will not work if both optional arguments of
% the \subfloat command are used. Furthermore, there needs to be a
% description of each subfigure *somewhere* and endfloat does not add
% subfigure captions to its list of figures. Thus, the best approach is to
% avoid the use of subfigure captions (many IEEE journals avoid them anyway)
% and instead reference/explain all the subfigures within the main caption.
% The latest version of endfloat.sty and its documentation can obtained at:
% http://www.ctan.org/pkg/endfloat
%
% The IEEEtran \ifCLASSOPTIONcaptionsoff conditional can also be used
% later in the document, say, to conditionally put the References on a 
% page by themselves.

% *** PDF, URL AND HYPERLINK PACKAGES ***
%
%\usepackage{url}
% url.sty was written by Donald Arseneau. It provides better support for
% handling and breaking URLs. url.sty is already installed on most LaTeX
% systems. The latest version and documentation can be obtained at:
% http://www.ctan.org/pkg/url
% Basically, \url{my_url_here}.

\usepackage{listings}

% *** Do not adjust lengths that control margins, column widths, etc. ***
% *** Do not use packages that alter fonts (such as pslatex).         ***
% There should be no need to do such things with IEEEtran.cls V1.6 and later.
% (Unless specifically asked to do so by the journal or conference you plan
% to submit to, of course. )

% correct bad hyphenation here
\hyphenation{op-tical net-works semi-conduc-tor}

==> sections/3_Overview.tex <==
\begin{figure*}[!htb]
  \begin{center}
  \includegraphics[width=0.98\textwidth]{img/fig_block_loop.png}
  \end{center}
  \caption{Block representation of the robotic system, its components, and its perception and control pipelines.}
  \label{fig:block_loop}
 \vspace{-12pt}
\end{figure*}

The core system consists of a robotic manipulator, an RGB camera, and an oxy-fuel torch (the end-effector).
The cutting control problem is formulated in the task space and is independent of the robot geometry.
In this work, however, the robot motions are simplified to focus on cutting control in isolation.
As such, the experimental setup consists of a robotic slider system for 1-D cuts.

\subsection{Oxy-fuel Torches and Combustion Cutting}
The cutting torch can be used to either burn the metal (combustion) or melt it (fusion), depending on the metal and on the fuel.
In oxy-propane cutting, carbon steel is burnt in a combustion reaction.
The cutting torch is fit with a tip (of a particular size) and connected to oxygen and fuel sources (at particular pressures).
The tip selection and pressure settings are configured before cutting based on the desired range of metal thickness to be cut.
A larger tip increases the maximum cutting thickness at the expense of higher pressures, which is wasteful at much smaller thicknesses.
The torch includes an oxygen bypass lever which when engaged increases the flow of oxygen (intensifies the combustion for more efficient cutting), and when released restores it.

Combustion cutting occurs as follows:
(1) The torch flame heats up the metal surface; this is called \textit{preheating}.
(2) When the local surface (the \textit{heat pool}) is hot enough, the oxygen bypass in engaged, the burning is accelerated, and the metal is cut.
(3) The torch is moved along the desired cutting path at an appropriate speed.

During cutting, the adequate shape, size, and temperature of the heal pool must be maintained by traversing at an adequate speed.
Traversing too quickly weakens the combustion, distorts the heat pool, and can extinguish it; all of which produce substandard or failed cuts.
Conversely, traversing too slowly is wasteful and yields poor surface texture where the cut can be resealed with slag due to excessive heat.
As such, the controller must move the torch at an appropriate speed along its cutting path, while (dis)engaging the bypass lever when appropriate.

\subsection{Robot Perception and Control}
For proper combustion cutting, the heat pool's properties (\textit{e.g.}, size, shape, and temperature) must stay within a desirable range.
In our vision-based approach, we use the \textit{heat pool quality} as a representative summary of the pool's geometric and thermal information relevant for combustion cutting.
In manual cutting, this ‘quality’ is intuitively determined by visually monitoring the pool's properties on the metal surface.
The robot can sense these environment states through its RGB camera. 
The resulting raw images are processed and simplified to filter out unnecessary information and noise. 
From these simplified images, the pool quality is estimated by computing the two quality metrics \textit{heat pool convexity} and \textit{heat pool intensity} as defined in section~\ref{sec:vision}. 
By using the quality estimate, the control algorithm determines the corresponding actions which in turn are implemented via the on-board controllers and actuators.
The robot thus updates the torch's motion along the reference cutting path, as well as the state of its oxygen bypass lever.

In our robotic setup, the camera is mounted at a fixed pose towards the torch tip.
The actuators are a stepper motor which sets the linear motion of the torch, and a linear actuator which (dis)engages the oxygen bypass. 
Using ROS~\cite{Quigley2009}, the system communications are distributed across a microcontroller for the low-level actuator control and a computer for image processing and high-level control actions. 
The computer is connected to the camera and the microcontroller, while the torch is connected to oxygen and propane tanks. 
The interaction of these components is summarized in Fig.~\ref{fig:block_loop}.

==> tables/algorithm_1.tex <==
\begin{algorithm}\label{alg:1}
\caption{TITLE}
\SetAlgoVlined
\SetKwInOut{KwInput}{Input}
\SetKwInOut{KwOutput}{Output}
\KwInput{Required input to the algorithm.}
\KwOutput{Expected output of the algorithm.}

 \textit{Comment given with pseudocode.}\\
 $\quad \mathtt{step}\;k \leftarrow 0$\\
 $\quad n_\mathsf{extremities} \leftarrow 0$\\
 $\quad {}^\mathsf{b}\mathrm{T}_{0} \leftarrow \mathtt{InitialViewpoint()}$\\
 
 \textit{Comment given with pseudocode.}\\
 \While{$n_\mathsf{extremities} < 2$}{
  \textit{Acquire, transform, concatenate, and filter clouds.}\\
  $\quad ({}^\mathsf{b}D_{\mathsf{total},k},\; {}^\mathsf{b}C_{k}) \leftarrow \mathtt{ProcessClouds}(k)$\\
  
  \textit{Comment given with pseudocode.}\\
  \eIf{$\operatorname{size}({}^\mathsf{b}D_{\mathsf{total},k}) - \operatorname{size}({}^\mathsf{b}D_{\mathsf{total},k-1}) \leq \delta_\mathsf{size}$}{
   $n_\mathsf{extremities} \leftarrow n_\mathsf{extremities} + 1$\\
    ${}^\mathsf{b}\mathrm{T}_{k+1} \leftarrow \mathtt{InitialViewpoint()}$\\
  }
  {
  \textit{Comment given with pseudocode.}\\
  $\mathtt{\quad Curve} \leftarrow  \mathtt{Fit}({}^\mathsf{b}D_{\mathsf{total},k},\; \mathtt{FittingMethod})$\\
  \textit{Comment given with pseudocode.}\\
   $\quad {}^\mathsf{b}\mathbf{d}_{k+1} \leftarrow \mathtt{Extrapolate}(\mathtt{Curve}, \; \delta_\mathsf{distance})$\\
   $\quad {}^\mathsf{b}\mathrm{R}_{k+1} \leftarrow \mathtt{GetNormalVec}({}^\mathsf{b}\mathbf{d}_{k+1},\; {}^\mathsf{b}C_{\mathsf{total},k})$\\
   $\quad {}^\mathsf{b}\mathrm{T}_{k+1} \leftarrow ({}^\mathsf{b}\mathbf{d}_{k+1},\; {}^\mathsf{b}\mathrm{R}_{k+1})$\\
  }
  $k \leftarrow k + 1$\\
 }
 \textbf{return} ${}^\mathsf{b}D_{\mathsf{total},k_\mathsf{stop}}$\\
\end{algorithm}

==> tables/table.tex <==
% https://www.tablesgenerator.com/
